STRIDE: An Open-Source, Low-Cost, and Versatile Bipedal Robot Platform for Research and Education

In this paper, we present STRIDE, a Simple, Terrestrial, Reconfigurable, Intelligent, Dynamic, and Educational bipedal platform. STRIDE aims to propel bipedal robotics research and education by providing a cost-effective implementation with step-by-step instructions for building a bipedal robotic platform while providing flexible customizations via a modular and durable design. Moreover, a versatile terrain setup and a quantitative disturbance injection system are augmented to the robot platform to replicate natural terrains and push forces that can be used to evaluate legged locomotion in practical and adversarial scenarios. We demonstrate the functionalities of this platform by realizing an adaptive step-to-step dynamics based walking controller to achieve dynamic walking. Our work with the open-soured implementation shows that STRIDE is a highly versatile and durable platform that can be used in research and education to evaluate locomotion algorithms, mechanical designs, and robust and adaptative controls.

==> ToDo.tex <==
\section{ToDo}
%%% Introduction
1. Compare with other Open source platforms 
\href{https://github.com/DRCL-USC/Hector_Simulation}{USC Biped}\\
(compare: hardware is not open-sourced\\
(inspiration: system and control architecture can mimic its figure \\
\href{https://github.com/RoboDesignLab/HOPPY-Project}{HOPPY jumping robot}\\
(compare: not a real bipedal robot, cannot be algorithm test bed\\
(inspiration:\\
\href{https://open-dynamic-robot-initiative.github.io/}{NYU dynamic robot initiative} \\
(compare:  4000 dollars, pure-3D printed, small load capacity, not so durable\\
(inspiration: choose open source protocol, learning its introduction writing method\\
\href{https://www.opensourceleg.org/about}{Umich open sourced leg}
(compare: \\
(inspiration: \\
Oncilla 
\href{https://ieeexplore.ieee.org/document/8794436/authors#authors}{Stanford-doggo}

\textbf{
1. Find all the papers or repos contain open-sourced robotic platforms.(\checkmark)\\
\indent 2. Compare and find our advantages.()\\
}

%%% Advantages
1. Low cost\\
2. versatile(education toolkit, research platform)\\
3. 2D -> for thoroughly evaluated algorithms, state of the art software architecture, \\
3. terrain(cheap \& versatile) and propeller(quantitative disturbance), modular system for other things. Design optimization. Off the shelf parts: no machining, but still durable. Customize repurpose the configuration or functionality of the robot.  \\
\textbf{1. Write out the mechanical design, electronics and software part of the paper(\checkmark)
2. Write out HLIP theory part of the paper
3. Write out Adaptive HLIP theory part of the paper 
4. Write out the introduction ()}


%%% Open Source Repo 
Open source: 
Mechanical design: BOM, CAD drawing,
Electrical: Wiring diagram
C++ repo, MATLAB simulator, 

%%% Experiments
\subsection{Experiments}

1. Rigid flat ground and step in place(if possible), velocity tracking

2. Terrain adaptation ( steady velocity on all granular terrains )

3. External disturbance (test the propeller(\checkmark))

4. design optimization (change leg inertia, leg length (both shin and thigh))


\begin{table}
    \centering
    \begin{tabular}{c|c|c|c}
       Category &  \\\hline 
       flat ground walking(velocity)  & 0.0m/s &  & \\\hline
       terrain adaptation  &  &  & \\\hline
       disturbance rejection  & 10N-h & 10N-v & 10N-(h+v)\\\hline
       design optimization  & 150 &  & \\\hline
    \end{tabular}
    \caption{Caption}
    \label{}
\end{table}

%%%% Detailed todo list
\textbf{\\
1. Design a new cover to cover all the wires(\checkmark)\\
2. A new more curved and wide contact foot(\checkmark)\\
3. Clean up the wire configuration for the boom and setup experiment place in the middle()\\
4. Renew step planning for legs.(\checkmark)\\
5. Test 4. in simulator(\checkmark)\\
6. Modify and print a new version of the foot, tire textures(\checkmark)\\
7. Add logic so robot will return to initial configuration after hanging in air.(\checkmark)}
\\


